Demand Estimation with Text and Image Data

We propose a demand estimation approach that leverages unstructured data to infer substitution patterns. Using pre-trained deep learning models, we extract embeddings from product images and textual descriptions and incorporate them into a mixed logit demand model. This approach enables demand estimation even when researchers lack data on product attributes or when consumers value hard-to-quantify attributes such as visual design. Using a choice experiment, we show this approach substantially outperforms standard attribute-based models at counterfactual predictions of second choices. We also apply it to 40 product categories offered on Amazon.com and consistently find that unstructured data are informative about substitution patterns.

==> implied_substitutes.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l c | l c | l c | l c}
\hline
Panel & Book & Prob. & Book & Prob. & Book & Prob. & Book & Prob. \\ \\hline
\multicolumn{8}{l}{\textbf{Please Tell Me (M)}} \\ \\hline
Please Tell Me (M) & 0.288 & Please Tell Me (M) & 0.154 & The Inmate (M) & 0.158 & The Inmate (M) & 0.178 \\ 
Please Tell Me (M) & 0.156 & The Inmate (M) & 0.145 & Serpent \& Wings (F) & 0.132 & The Housemaid (M) & 0.137 \\ 
Please Tell Me (M) & 0.32 & Please Tell Me (M) & 0.168 & Please Tell Me (M) & 0.199 & Please Tell Me (M) & 0.197 \\ 
Please Tell Me (M) & 0.093 & Don't Believe (S) & 0.141 & Don't Believe (S) & 0.113 & Court of Ravens (F) & 0.126 \\ 
Please Tell Me (M) & 0.08 & Dopamine Detox (S) & 0.116 & The Ritual (M) & 0.105 & Court of Ravens (F) & 0.108 \\ 
Please Tell Me (M) & 0.106 & The Housemaid (M) & 0.152 & The Inmate (M) & 0.15 & The Inmate (M) & 0.166 \\ 
Please Tell Me (M) & 0.112 & The Housemaid (M) & 0.141 & Please Tell Me (M) & 0.152 & Please Tell Me (M) & 0.129 \\ 
Please Tell Me (M) & 0.096 & The Inmate (M) & 0.145 & The Housemaid (M) & 0.142 & Please Tell Me (M) & 0.146 \\ 
Please Tell Me (M) & 0.079 & Dopamine Detox (S) & 0.133 & The Housemaid (M) & 0.125 & The Housemaid (M) & 0.103 \\ 
\hline
\multicolumn{8}{l}{\textbf{The Inmate (M)}} \\ \\hline
The Inmate (M) & 0.293 & The Inmate (M) & 0.158 & Please Tell Me (M) & 0.184 & Please Tell Me (M) & 0.211 \\ 
The Inmate (M) & 0.167 & Please Tell Me (M) & 0.166 & Please Tell Me (M) & 0.191 & Please Tell Me (M) & 0.162 \\ 
The Inmate (M) & nan & nan & nan & nan & nan & nan & nan \\ 
The Inmate (M) & 0.117 & Dopamine Detox (S) & 0.144 & Please Tell Me (M) & 0.144 & The Inmate (M) & 0.146 \\ 
The Inmate (M) & 0.105 & The Inmate (M) & 0.153 & The Housemaid (M) & 0.134 & The Housemaid (M) & 0.123 \\ 
The Inmate (M) & 0.105 & The Inmate (M) & 0.126 & Don't Believe (S) & 0.138 & Don't Believe (S) & 0.09 \\ 
The Inmate (M) & 0.094 & Don't Believe (S) & 0.137 & Art of Letting Go (S) & 0.135 & The Inmate (M) & 0.125 \\ 
The Inmate (M) & 0.087 & The Housemaid (M) & 0.129 & The Inmate (M) & 0.135 & The Inmate (M) & 0.122 \\ 
The Inmate (M) & 0.084 & Don't Believe (S) & 0.14 & Dopamine Detox (S) & 0.166 & Please Tell Me (M) & 0.156 \\ 
\hline
\multicolumn{8}{l}{\textbf{The Housemaid (M)}} \\ \\hline
The Housemaid (M) & nan & nan & nan & nan & nan & nan & nan \\ 
The Housemaid (M) & 0.148 & Dopamine Detox (S) & 0.126 & The Inmate (M) & 0.126 & The Inmate (M) & 0.135 \\ 
The Housemaid (M) & 0.268 & Don't Believe (S) & 0.154 & Don't Believe (S) & 0.138 & The Housemaid (M) & 0.153 \\ 
The Housemaid (M) & 0.068 & Art of Letting Go (S) & 0.092 & Art of Letting Go (S) & 0.087 & Dopamine Detox (S) & 0.093 \\ 
The Housemaid (M) & 0.07 & Art of Letting Go (S) & 0.1 & Don't Believe (S) & 0.093 & Dopamine Detox (S) & 0.092 \\ 
The Housemaid (M) & 0.075 & Serpent \& Wings (F) & 0.105 & Art of Letting Go (S) & 0.095 & Art of Letting Go (S) & 0.085 \\ 
The Housemaid (M) & 0.057 & Serpent \& Wings (F) & 0.095 & The Housemaid (M) & 0.132 & The Housemaid (M) & 0.1 \\ 
The Housemaid (M) & 0.056 & Art of Letting Go (S) & 0.1 & Art of Letting Go (S) & 0.124 & The Housemaid (M) & 0.112 \\ 
The Housemaid (M) & 0.08 & The Housemaid (M) & 0.138 & The Inmate (M) & 0.136 & The Inmate (M) & 0.141 \\ 
\hline

\end{tabular}
\caption{Predicted second-choice probabilities and their data counterparts.}
\label{tab:implied_substitutes}
\end{table}

